Lightweight, Practical Encrypted Face Recognition with GPU Support

Face recognition typically operates in a client-server setting, where the client extracts a compact face embedding and the server performs similarity search over a template database. Since facial data is highly sensitive, this raises significant privacy concerns. Fully homomorphic encryption (FHE) addresses these concerns by enabling end-to-end encrypted similarity search. However, existing FHE-based protocols are computationally costly and, especially, impose high memory overhead due to large rotation-key sets and bandwidth-bound homomorphic operations. Building on prior work, HyDia (PoPETS 2025), we introduce algorithmic and system-level improvements targeting real-world deployment with resource-constrained (edge) clients. First, we propose BSGS-Diagonal, a fast and memory-efficient similarity computation algorithm that applies a Baby-Step/Giant-Step strategy with precomputed rotations reused across consecutive matrix--vector products. This yields a 91% reduction in rotation keys (~14GB less client memory) and cuts peak server-side CPU RAM usage from over 33GB to 11GB for databases up to 1M entries, with runtime improvements of up to 1.57x for membership verification and 1.43x for identification. Second, we introduce GPU-optimized similarity computation kernels, including an efficient homomorphic Chebyshev evaluator built upon FIDESlib (ISPASS 2025), a CKKS-level GPU library based on OpenFHE. Rather than offloading individual CKKS primitives, our integrated kernels fuse operations to avoid repeated CPU--GPU ciphertext movement and costly FIDESlib/OpenFHE data-structure conversions. Our HyDia and BSGS GPU results achieve up to 9x and 21x speedups on single GPU (and up to 287x and 211x using multi-GPUs), respectively, enabling sub-second encrypted face recognition for databases up to 2^16 entries (or 2^19 entries in a multi-GPU setting), while further reducing host memory usage.

==> hydia_shorter.tex <==
HyDia is a three-party CKKS-based protocol for one-to-many ($1{:}K$) facial matching where both query and database embeddings are encrypted end-to-end, supporting membership verification and identification. An enroller performs a one-time setup, extracting, preprocessing, encrypting, and uploading database template ciphertexts to the server, after which the server homomorphically evaluates encrypted queries submitted by the client. Figure~\ref{fig:hydia} illustrates the protocol and the entities involved.

\input{figure_protocol.tex}

HyDia's design avoids revealing per-entry similarity scores by returning only a thresholded match decision or matching indices, preventing a semi-honest client from learning additional database information. It outperforms prior methods~\cite{ibarrondo2023grote,choi2024blind,engelsma2022hers} by adapting diagonalized matrix multiplication to the $1{:}K$ scenario (reducing HE overhead and enabling higher parallelism) and by supporting single-ciphertext queries rather than hundreds of ciphertexts per query, significantly reducing communication. It also uses a hybrid polynomial thresholding approximation combining a low-depth Chebyshev approximation with a fixed-degree polynomial from~\cite{cheon2020efficient}, improving accuracy near the decision boundary without increasing multiplicative depth.
